All the World's a (Hyper)Graph: A Data Drama

We introduce Hyperbard, a dataset of diverse relational data representations derived from Shakespeare's plays. Our representations range from simple graphs capturing character co-occurrence in single scenes to hypergraphs encoding complex communication settings and character contributions as hyperedges with edge-specific node weights. By making multiple intuitive representations readily available for experimentation, we facilitate rigorous representation robustness checks in graph learning, graph mining, and network analysis, highlighting the advantages and drawbacks of specific representations. Leveraging the data released in Hyperbard, we demonstrate that many solutions to popular graph mining problems are highly dependent on the representation choice, thus calling current graph curation practices into question. As an homage to our data source, and asserting that science can also be art, we present all our points in the form of a play.

==> text/checklist.tex <==
% !TeX spellcheck = en_US
% !TeX root = ../main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%	justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%	\item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes{The main contribution is the \ourdata dataset, which is fully documented in the Appendix and made freely available along with the code generating it, see \cite{coupette2022hyperdata} and \cite{coupette2022hypercode}.}
		\item Did you describe the limitations of your work?
		\answerYes{See the dataset documentation in the Appendix.}
		\item Did you discuss any potential negative societal impacts of your work?
		\answerYes{See the dataset documentation in the Appendix.}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{See the dataset documentation in the Appendix.}
	\end{enumerate}
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerNA{The paper does not include theoretical results.}
		\item Did you include complete proofs of all theoretical results?
		\answerNA{See comment on 2.(a).}
	\end{enumerate}
	
	\item If you ran experiments (e.g. for benchmarks)...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerYes{See the dataset documentation in the Appendix as well as \cite{coupette2022hyperdata} and \cite{coupette2022hypercode}.}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerNA{Our experiments do not involve model training.}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerNA{All experimental results shown are deterministic.}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerYes{See the dataset documentation in the Appendix.}
	\end{enumerate}
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerYes{See \cite{folger2022} and the dataset documentation in the Appendix.}
		\item Did you mention the license of the assets?
		\answerYes{See the dataset documentation in the Appendix.}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerYes{See \cite{coupette2022hyperdata} and \cite{coupette2022hypercode}.}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerYes{See the dataset documentation in the Appendix.}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerYes{See the dataset documentation in the Appendix.}
	\end{enumerate}
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{We did not use crowdsourcing or conduct research with human subjects.}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{See comment on 5.(a).}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{See comment on 5.(a).}
	\end{enumerate}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> text/fourth.tex <==
% !TeX spellcheck = en_US
% !TeX root = ../main.tex
%\begin{figure}[h]\small
%	\hspace*{-2em}\begin{tabular}[t]{rp{0.5\linewidth}|}
%		\phantomsection\addcontentsline{toc}{section}{Act IV}
%		\pls{\hfil\textsc{Act IV.}}
%		\pls{\hfil\textsc{Scene I.}---The Community.}
%	\end{tabular}
%	\begin{tabular}[t]{rp{0.5\linewidth}}
%	\end{tabular}
%\end{figure}

%
%adapt sun/moon exchange scientist/raw data
%
%Why sir, I trust I may have leave to speak,
%And speak I will. I am no child, no babe;
%Your betters have endured me say my mind,
%And if you cannot, best you stop your ears.
%My tongue will tell the anger of my heart,
%Or else my heart concealing it will break,
%And rather than it shall, I will be free
%Even to the uttermost, as I please, in words.
%(4.3.74–80)
%
%And be it the moon, or sun, or what you please;
%And if you please to call it a rush-candle,
%Henceforth I vow it shall be so for me
%...
%But sun it is not, when you say it is not,
%And the moon changes even as your mind:
%What you will have it named, even that it is,
%And so it shall be so for Katherine.
%(4.5.12–15; 4.5.19–22)
